Monitoring Browsing Behavior of Customers in Retail Stores via RFID Imaging

In this paper, we propose to use commercial off-the-shelf (COTS) monostatic RFID devices (i.e. which use a single antenna at a time for both transmitting and receiving RFID signals to and from the tags) to monitor browsing activity of customers in front of display items in places such as retail stores. To this end, we propose TagSee, a multi-person imaging system based on monostatic RFID imaging. TagSee is based on the insight that when customers are browsing the items on a shelf, they stand between the tags deployed along the boundaries of the shelf and the reader, which changes the multi-paths that the RFID signals travel along, and both the RSS and phase values of the RFID signals that the reader receives change. Based on these variations observed by the reader, TagSee constructs a coarse grained image of the customers. Afterwards, TagSee identifies the items that are being browsed by the customers by analyzing the constructed images. The key novelty of this paper is on achieving browsing behavior monitoring of multiple customers in front of display items by constructing coarse grained images via robust, analytical model-driven deep learning based, RFID imaging. To achieve this, we first mathematically formulate the problem of imaging humans using monostatic RFID devices and derive an approximate analytical imaging model that correlates the variations caused by human obstructions in the RFID signals. Based on this model, we then develop a deep learning framework to robustly image customers with high accuracy. We implement TagSee scheme using a Impinj Speedway R420 reader and SMARTRAC DogBone RFID tags. TagSee can achieve a TPR of more than ~90% and a FPR of less than ~10% in multi-person scenarios using training data from just 3-4 users.

==> Kamran/RTI_brief.tex <==
\presec
\section{Related Work}

\textbf{Radio Tomographic Imaging:}
Radio Tomographic Imaging (RTI) is a technology for ``imaging'' attenuations caused by humans or other physical objects in RF signals between different nodes of a wireless network. An RTI system consists of multiple wireless nodes capable of transmitting and receiving independently. For $K$ wireless nodes, there are $M = K(K-1)/2$ unique links in an RTI system. Usually, round robin or token passing based algorithms are used, so that each link can operate by taking turns and without creating interference in the transmission of any other node. In each RTI system, the area being ``imaged'' is divided into $N$ different \textit{voxels} (just like \textit{pixels} in an image), and the goal is to image the attenuations occurring in different voxels, leading to localization of objects causing those attenuations. 

There has been a more recent work which uses bi-static RFID readers (separate receive and transmit antennas), instead of a sensor node network, for RTI based device free localization \cite{wagner2012passive}. Their problem is exactly similar to the one of their previous RTI works \cite{wilson2010radio}, and therefore, they build upon their previous RTI work to perform RTI using bi-static RFIDs. Although, we use similar RTI techniques as used in the aforementioned previous works \cite{wilson2010radio,wagner2012passive} (especially, our image calculation approach is based on the original one in \cite{wilson2010radio}), yet our scheme differs from previous ones in following terms:

\begin{enumerate}
	\item Our purpose of using RTI is not device free localization. Currently, we are only interested in monitoring shelves in retail stores, for example, counting the number of customers coming to a specific shelve.
	\item We use mono-static RFID readers instead of bi-static readers (which have separate transmit and receive antennas).
	\item We use inherent frequency hopping capability of RFID communication and phase information provided by commodity RFID readers for reducing effect of multipaths in our monitoring system.
	\item We propose an automatic way of tuning the weight matrix specific to our application, which is used in image reconstruction part of our technique. The weight matrix changes according to the dynamically changing RF channel between the RFID reader and the deployed tags.
	\item We improve the image reconstruction results by using multiple priors related to the variation of received signal strength (RSS) of backscattered signals across the image plane between a mono-static RFID reader and deployed RFID tags.
	\item Reduction in multipath effect by utilizing frequency hopping and accurate phase information capabilities of monostatic RFID readers system, on top of the real-time calibration of weight matrix, makes our system capable of tracking multiple people at the same time. We use previously proposed \textit{blob} tracking algorithms to track and count blobs in the RTI images created due to human motion.
\end{enumerate}

The basic part of every RTI scheme is to model the changes in attenuation happening inside the area being monitored using the signal strength measurements made at several different nodes of the RTI network. Moreover, as motion of an object in an RTI area creates multipaths, the noise in such a dynamic multipath environment also needs to be modeled. In order to achieve this goal, the authors represent the signal strength of a link $i$ as:
\vspace{-0.05in}
\begin{equation}
y_i(t) = P_i - L_i - S_i(t) - F_i(t) - v_i(t)
\end{equation}

where $P_i$ is transmit power (dB), $S_i$ is shadowing loss due to objects, $F_i(t)$ is loss due to fading, $L_i$ are \textit{static} losses (related to distance, antenna patterns, device inconsistencies, etc.) and $v_i$ is measurement noise. Moreover, shadowing loss $S_i$ for a certain link for a specific time is expressed in terms of attenuation caused in all the voxels as:
\vspace{-0.05in}
\begin{equation}
S_i(t) = \sum_{j=1}^{N} w_{ij}x_j(t)
\end{equation}

where $x_j(t)$ is attenuation at voxel $j$ at anytime $t$ and $w_{ij}$ is weight-age or contribution of voxel $j$ towards attenuation of link $i$. In order to simplify the problem, authors propose to image only the \textit{changing attenuations} between two different times and group the fading and measurement noise into one vector $\mathbf{n}$. The changes in RSS of different links ($\mathbf{y}$) are then written in terms of the attenuations ($\mathbf{x}$) and an $M \times N$ weight matrix ($\mathbf{W}$) specifying the weight-age of attenuations cause in different voxels corresponding to different links as:
\vspace{-0.05in}
\begin{equation}
 \mathbf{y} = \mathbf{W} \mathbf{x} + \mathbf{n}
\label{eqn:optimzation1}
\end{equation}

The next steps are a) finding a reasonable and effective linear \textit{weight model} which can represent the weight matrix $\mathbf{W}$ and b) modeling noise. 

a) In order to model weight matrix, the authors propose to use a statistical model to describe linear effect of ``attenuation field'' on path loss of different links. In order to determine weights of different voxels in the area, they use an imaginary ellipsoid centered (Fresnel Zone) at the locations of different RF nodes in the network. \textit{The intuition is that ellipsoids will be determining the LOS path of each respective link. If a voxel is within the LOS of a link, it will be assigned more weight as compared to the voxel which does not fall in LOS.} If a voxel is outside the ellipsoid, the assigned weight is 0. However, if the voxel is inside the ellipsoid, the assigned weight is inversely proportional to square root of the distance. \textit{This is because the signals between longer links reflect and diffract around the object being tracked, thus providing less information about the changes in attenuation as compared to a short link.} Let $d$ be distance between two nodes of a certain link $i$, $d_{ij}(1)$ and $d_{ij}(2)$ be distance from center of voxel $j$ to the two nodes of the link $i$ and $\Theta$ be a parameter describing ellipsoid's width. Then the weights can be modeled as:
\vspace{-0.05in}
\[
w_{ij}= 
\begin{cases}
\frac{1}{\sqrt{d}},& \text{if } d_{ij}(1) + d_{ij}(2) < d + \Theta\\
0,              & \text{otherwise}
\end{cases}
\]

$\lambda$ is usually chosen so that only the voxels corresponding to line-of-sight (LOS) path are considered. 

b) After modeling of weights for different voxels corresponding to different links, authors propose to model noise as a two-part \textit{log-normal mixture model}. \textit{The reason behind using this model is the similarity of the log-normal distribution with the logarithm of a Rician random variable (often used to model effects of fading in wireless channels)}. 

The authors also derive an error bounds for their proposed models for attenuation weight-age of different voxels corresponding to different links and noise. 

In order to re-construct image from the RSS values obtained from all the links, the most straightforward way is to calculate the least-squares solution for the equation \ref{eqn:optimzation1} like this (for simplification, we can take $\bigtriangleup x = x$ and $\bigtriangleup y = y$):

\vspace{-0.1in}
\begin{equation}
\mathbf{x_{LS}} = (\mathbf{W}^T\mathbf{W})^{-1}\mathbf{W}^T \mathbf{y}
\label{eqn:solution1}
\end{equation}

However, the matrix $\mathbf{W}$ is not full rank in case of RTI systems, which makes RTI an \textit{ill-posed inverse problem}. In order to handle ill-posedness, the authors propose to use \textit{Tikhonov Regularization} for minimization of the objective function of the original problem (i.e. represented by equation \ref{eqn:optimzation1}). The objective function to be minimized becomes:
\vspace{-0.05in}
\begin{equation}
f(\mathbf{x}) = \frac{1}{2}||\mathbf{Wx-y}||^2 + \alpha(||\mathbf{D}_X\mathbf{x}||^2 + ||\mathbf{D}_Y\mathbf{y}||^2)
\label{eqn:minimization1}
\end{equation}

where $\mathbf{D}_X$ and $\mathbf{D}_Y$ are different operators in X and Y directions respectively. The solution comes out to be:
\vspace{-0.05in}
\begin{equation}
\mathbf{\hat{x}} = (\mathbf{W}^T\mathbf{W} + \alpha(\mathbf{D}_X^T\mathbf{D}_X + \mathbf{D}_Y^T\mathbf{D}_Y))^{-1}\mathbf{W}^T \mathbf{y}
\label{eqn:solution2}
\end{equation}

The total number of multiplications involved in image reconstruction procedure are $\frac{N\times K(K-1)}{2}$, where $N$ = number of voxels and $K$ = number of nodes. The authors have also used the inverse of the covariance matrix $\mathbf{C_x}$ of $\mathbf{\hat{x}}$ as a prior in the technical report of their paper.
\vspace{-0.05in}
\begin{equation}
\mathbf{\hat{x}} = (\mathbf{W}^T\mathbf{W} + \mathbf{C_x}^{-1})^{-1}\mathbf{W}^T \mathbf{y}
\label{eqn:solution3}
\end{equation}
 We will discuss later on how we use a combination of these priors to improve our image reconstruction results.
 
\textbf{Passive RFID tomographic imaging for device-free user localization\cite{wagner2012passive}:} This work is very similar to the aforementioned work, and builds on exactly the same techniques. However, authors have used bi-static RFID network (as shown in figure \ref{fig:difference}) in this particular work, where transmitting and receiving antennas are deployed on two opposites sides of the area being monitored for device free localization, and RFID tags/transponders are deployed in between. RTI is performed as human moves between the space spanned by TX antennas, RX antennas and the RFID tags, creating disturbance between each of the the TX-Tag-RX links. They use different weights for forward (TX-Tag) link and backward (RX-Tag) links, which are tunable with different values of $\Theta$ for the elliptical Fresnel zones corresponding to each different link. Figure \ref{fig:rfid_rti} shows an example~\cite{wagner2012passive} taken from their paper. This technique has a serious scalability issue, because both TX and RX antennas have to be connected with the same receiver and may need longer wires in scenarios where a larger area is required to be monitored.

\begin{figure}[!t]
	\centering
	\captionsetup{justification=centering}
	%	\subfigure[ \noindent{Tonemap N1-N2}]{
	%		\label{fig:illustration}
	\includegraphics[width=0.4\textwidth]{figures/rfid_rti.pdf}%}
	\vspace{-0.1in}
	\caption{RFID based RTI example \cite{wagner2012passive}} % Tonemaps (Location C and D)
	\label{fig:rfid_rti}
	\vspace{-0.15in}
\end{figure}

==> Kamran/RTIprimer.tex <==
\section{Primer}
\presec

\subsection{RFIDs}
\vspace{-0.05in}

\vspace{-0.05in}
\subsection{Radio Tomographic Imaging (RTI)}
\vspace{-0.05in}
The basic part of every RTI scheme is to model the changes in attenuation happening inside the area being monitored using the signal strength measurements made at several different nodes of the RTI network. Moreover, as motion of an object in an RTI area creates multipaths, the noise in such a dynamic multipath environment also needs to be modeled. In order to achieve this goal, the authors represent the signal strength of a link $i$ as:
\vspace{-0.05in}
\begin{equation}
y_i(t) = P_i - L_i - S_i(t) - F_i(t) - v_i(t)
\end{equation}

where $P_i$ is transmit power (dB), $S_i$ is shadowing loss due to objects, $F_i(t)$ is loss due to fading, $L_i$ are \textit{static} losses (related to distance, antenna patterns, device inconsistencies, etc.) and $v_i$ is measurement noise. Moreover, shadowing loss $S_i$ for a certain link for a specific time is expressed in terms of attenuation caused in all the voxels as:
\vspace{-0.05in}
\begin{equation}
S_i(t) = \sum_{j=1}^{N} w_{ij}x_j(t)
\end{equation}

where $x_j(t)$ is attenuation at voxel $j$ at anytime $t$ and $w_{ij}$ is weight-age or contribution of voxel $j$ towards attenuation of link $i$. In order to simplify the problem, authors propose to image only the \textit{changing attenuations} between two different times and group the fading and measurement noise into one vector $\mathbf{n}$. The changes in RSS of different links ($\mathbf{y}$) are then written in terms of the attenuations ($\mathbf{x}$) and an $M \times N$ weight matrix ($\mathbf{W}$) specifying the weight-age of attenuations cause in different voxels corresponding to different links as:
\vspace{-0.05in}
\begin{equation}
\mathbf{y} = \mathbf{W} \mathbf{x} + \mathbf{n}
\label{eqn:optimzation1}
\end{equation}

The next steps are a) finding a reasonable and effective linear \textit{weight model} which can represent the weight matrix $\mathbf{W}$ and b) modeling noise. 

a) In order to model weight matrix, the authors propose to use a statistical model to describe linear effect of ``attenuation field'' on path loss of different links. In order to determine weights of different voxels in the area, they use an imaginary ellipsoid centered (Fresnel Zone) at the locations of different RF nodes in the network. \textit{The intuition is that ellipsoids will be determining the LOS path of each respective link. If a voxel is within the LOS of a link, it will be assigned more weight as compared to the voxel which does not fall in LOS.} If a voxel is outside the ellipsoid, the assigned weight is 0. However, if the voxel is inside the ellipsoid, the assigned weight is inversely proportional to square root of the distance. \textit{This is because the signals between longer links reflect and diffract around the object being tracked, thus providing less information about the changes in attenuation as compared to a short link.} Let $d$ be distance between two nodes of a certain link $i$, $d_{ij}(1)$ and $d_{ij}(2)$ be distance from center of voxel $j$ to the two nodes of the link $i$ and $\Theta$ be a parameter describing ellipsoid's width. Then the weights can be modeled as:
\vspace{-0.05in}
\[
w_{ij}= 
\begin{cases}
\frac{1}{\sqrt{d}},& \text{if } d_{ij}(1) + d_{ij}(2) < d + \Theta\\
0,              & \text{otherwise}
\end{cases}
\]

$\lambda$ is usually chosen so that only the voxels corresponding to line-of-sight (LOS) path are considered. 

b) After modeling of weights for different voxels corresponding to different links, authors propose to model noise as a two-part \textit{log-normal mixture model}. \textit{The reason behind using this model is the similarity of the log-normal distribution with the logarithm of a Rician random variable (often used to model effects of fading in wireless channels)}. 

The authors also derive an error bounds for their proposed models for attenuation weight-age of different voxels corresponding to different links and noise. 

In order to re-construct image from the RSS values obtained from all the links, the most straightforward way is to calculate the least-squares solution for the equation \ref{eqn:optimzation1} like this (for simplification, we can take $\bigtriangleup x = x$ and $\bigtriangleup y = y$):

\vspace{-0.1in}
\begin{equation}
\mathbf{x_{LS}} = (\mathbf{W}^T\mathbf{W})^{-1}\mathbf{W}^T \mathbf{y}
\label{eqn:solution1}
\end{equation}

However, the matrix $\mathbf{W}$ is not full rank in case of RTI systems, which makes RTI an \textit{ill-posed inverse problem}. In order to handle ill-posedness, the authors propose to use \textit{Tikhonov Regularization} for minimization of the objective function of the original problem (i.e. represented by equation \ref{eqn:optimzation1}). The objective function to be minimized becomes:
\vspace{-0.05in}
\begin{equation}
f(\mathbf{x}) = \frac{1}{2}||\mathbf{Wx-y}||^2 + \alpha(||\mathbf{D}_X\mathbf{x}||^2 + ||\mathbf{D}_Y\mathbf{y}||^2)
\label{eqn:minimization1}
\end{equation}

where $\mathbf{D}_X$ and $\mathbf{D}_Y$ are different operators in X and Y directions respectively. The solution comes out to be:
\vspace{-0.05in}
\begin{equation}
\mathbf{\hat{x}} = (\mathbf{W}^T\mathbf{W} + \alpha(\mathbf{D}_X^T\mathbf{D}_X + \mathbf{D}_Y^T\mathbf{D}_Y))^{-1}\mathbf{W}^T \mathbf{y}
\label{eqn:solution2}
\end{equation}

The total number of multiplications involved in image reconstruction procedure are $\frac{N\times K(K-1)}{2}$, where $N$ = number of voxels and $K$ = number of nodes. The authors have also used the inverse of the covariance matrix $\mathbf{C_x}$ of $\mathbf{\hat{x}}$ as a prior in the technical report of their paper.
\vspace{-0.05in}
\begin{equation}
\mathbf{\hat{x}} = (\mathbf{W}^T\mathbf{W} + \mathbf{C_x}^{-1})^{-1}\mathbf{W}^T \mathbf{y}
\label{eqn:solution3}
\end{equation}
We will discuss later on how we use a combination of these priors to improve our image reconstruction results.

\textbf{Passive RFID tomographic imaging for device-free user localization\cite{wagner2012passive}:} This work is very similar to the aforementioned work, and builds on exactly the same techniques. However, authors have used bi-static RFID network in this particular work, where transmitting and receiving antennas are deployed on two opposites sides of the area being monitored for device free localization, and RFID tags/transponders are deployed in between. RTI is performed as human moves between the space spanned by TX antennas, RX antennas and the RFID tags, creating disturbance between each of the the TX-Tag-RX links. They use different weights for forward (TX-Tag) link and backward (RX-Tag) links, which are tunable with different values of $\Theta$ for the elliptical Fresnel zones corresponding to each different link. Figure \ref{fig:rfid_rti} shows an example~\cite{wagner2012passive} taken from their paper. This technique has a serious scalability issue, because both TX and RX antennas have to be connected with the same receiver and may need longer wires in scenarios where a larger area is required to be monitored.

%\begin{figure}[!t]
%	\centering
%	\captionsetup{justification=centering}
%	%	\subfigure[ \noindent{Tonemap N1-N2}]{
%	%		\label{fig:illustration}
%	\includegraphics[width=0.4\textwidth]{figures/rfid_rti.pdf}%}
%	\vspace{-0.1in}
%	\caption{RFID based RTI example \cite{wagner2012passive}} % Tonemaps (Location C and D)
%	\label{fig:rfid_rti}
%	\vspace{-0.15in}
%\end{figure}

==> Kamran/discussion.tex <==
\section{Discussion}

==> Kamran/maqbooloverview.tex <==
\presec
\section{Maqbool Overview}
\vspace{-0.05in}
[Still working]
%
To image human obstructions while customers browse product categories in front of a shelf, \textit{Maqbool} needs to have an image reconstruction model of how customers cause variations in RFID signals as they browse. 
%
\textit{Maqbool} builds RTI models for imaging multiple customers browsing different products, in the following five steps.

%The first step is noise removal, where GEAT passes the
%time series of touch point coordinates in each gesture sample
%through a filter to remove high frequency noise.
%
%The second step is feature extraction, where GEAT extracts
%the values of the seven types of features from the gesture
%samples and concatenates these values to form a feature
%vector. To extract feature values of velocity magnitude, velocity
%direction, and device accelerations, GEAT segments
%each stroke in a gesture sample into sub-strokes at multiple
%time resolutions and extracts values from these sub-strokes.
%We call these three types of features sub-stroke based features.
%For the remaining four types of features, GEAT extracts
%values from the entire strokes in each gesture. We call
%these four types of features stroke based features.
%
%The third step is feature selection. For each feature element,
%GEAT first partition all its N values, where N is the
%total number of training samples, into the least number of
%minimum variance partitions, where the coefficient of variation
%for each partition is below a threshold. If the number
%of minimum variance partitions is less than or equal to the
%number of postures in which the legitimate user provided
%the training samples, then we select this feature element;
%otherwise, we discard it. For this purpose, ideally the user
%should inform GEAT the number of postures in which he
%performed the training gestures. However, if the user does
%not provide this information, the classification accuracy of
%GEAT decreases, but only very slightly, as shown in our
%experimental results in Section 9.
%
%The fourth step is classifier training. GEAT first partitions
%all N feature vectors into the minimum number of groups
%so that within each group, all feature vectors belong to the
%same minimum variance partition for any feature element.
%We call each group a consistent training group. Then, for
%each group of feature vectors, GEAT builds a model in the
%form of an ensemble of SVDE classifiers trained using these
%vectors. Note that we do not use any gestures from imposters
%in training GEAT because in the real-world deployment of
%authentication systems, training samples are typically available
%only from the legitimate user.
%
%The fifth step is gesture ranking. For each gesture, GEAT
%repeats the above four steps and then ranks the gestures
%based on their EERs. A user can pick 1 ≤ n ≤ 10 gestures
%to be used in each user authentication. Although the larger
%n is, the higher accuracy GEAT has, for practical purposes
%such as unlocking smart phone screens, n = 1 (or 3 at most)
%gives us high enough accuracy. To calculate the EER of a
%gesture, GEAT needs the true positive rates (TPR) and false
%positive rates (FPR) for that gesture. TPRs for each gesture
%are calculated using 10 fold cross validation on legitimate
%user’s samples of the gesture. To calculate FPRs, GEAT
%needs imposter samples, which are not available in real world
%deployment at the time of training. Therefore, GEAT generates
%synthetic imposter samples by elastically deforming the
%samples of legitimate user using cubic B-splines and calculates
%the FPRs using these synthetic imposter samples. Note
%that the synthetic imposter samples are used only in ranking
%gestures, the performance evaluation of GEAT that we
%present in Section 9 is done entirely on real world imposter
%samples. These synthetic imposter samples are not used in
%classifier training either.

%Table 1 summarizes the symbols used in this paper.

==> Kamran/primer.tex <==
%\presec
\subsection{Primer} \label{sec:overview}
%\vspace{-0.05in}
In this section, we briefly give an overview of the monostatic RFID technology, and introduce the parameters, i.e. RSS and Phase, which SeeWSee's algorithms use for effective image reconstruction. 
%
We also introduce fundamentals of our baseline RF imaging approach for our mono-static RFID system, which forms the basis of our proposed \textit{deep neural networks} based imaging technique.

%\vspace{-0.05in}
\subsubsection{Monostatic RFIDs}
%\vspace{-0.05in}
%
In a typical monostatic RFID system, a \textit{reader} transmits continuous wave signals to interrogate tags deployed in its proximity, and then receives backscattered signals from those tags which contain their unique IDs.
%
We use industrial standard, EPC Global Class 1 Generation 2 (C1G2) RFID \cite{epcglobal2008radio} compatible, Ultra-High-Frequency (UHF) monostatic RFID tags and readers in our proposed popularity tracking scheme.
%
The RFID readers we use operate in the frequency range 902-928 MHz, through a \textit{frequency hopping} (FH) mechanism, where the frequency range is divided into 50 subcarriers (i.e. 902.75 - 927.25 MHz with an interval of 0.25 MHz), which are randomly hopped between during each interrogation cycle. 
%
This FH capability reduces interference between nearby RFID readers, and leads to robust and reliable interrogation of tags in cases where some part of the spectrum is under fade.
%
Also, these readers are equipped with multiple antennas, where query-response communication corresponding to each antenna is multiplexed in time, where each antenna interrogates the tags in an alternating manner.
%
In each query-response communication, the EPC C1G2 compatible RFID tags respond to RFID signals from a reader, through a random access collision avoidance technique called \textit{slotted} ALOHA \cite{kawakita2006anti}.
%
For this work, we have used Impinj Speedway R420 RFID readers, which are capable of reading upto $\sim 450~tags/s$, which allows for gathering enough RSS and phase information from the deployed tags, required for smoother and near real-time popularity tracking.
%\vspace{-0.05in}
\subsubsection{Received Signal Strength (RSS)}
%\vspace{-0.05in}

Monostatic RFID channel is a double fading channel, i.e. each fade is experienced twice, once in the forward link and once in the reverse link.
%
A typical RFID use case scenario involves indoor multipath environment, where each link consists of a line-of-sight (LOS) path and a few major reflections.
%
For Mono-static RFID readers, for a given subcarrier of wavelength $\lambda$, the received power $P_{r,k,a}$ at the reader antenna $a$, of the backscattered signal from tag $k$ located at distance $d$ from the reader, can be approximated in terms of transmit power $P_{t}$ for a free space scenario as:
\vspace{-0.05in}
\begin{equation*}
P_{r,k,a} = P_{t} G_a^2 G_{k}^2 T_{b,k} \cdot (\frac{\lambda}{4\pi d})^4
\label{eqn:solution4}
\vspace{-0.05in}
\end{equation*}

where $G_{a}$ and $G_k$ are $a^{th}$ reader antenna and $k^{th}$ tag antenna gains, respectively. $T_{b,k}$ is the backscatter or modulation loss of the $k^{th}$ tag. Next, we assume that $P_{t}$, $G_k$, $G_a$ and $T_{b,k}$ remain constant for a tag-antenna pair, and then re-write the simplified logarithmic form of above equation, which we use later on, while formulating a baseline RTI approach in \S \ref{sec:popularitytracking}, for our monostatic RFID system :
\vspace{-0.05in}
\begin{equation}
RSS_k~(dBm) = A_{0,k} + 10 \cdot \beta_k\log[(\frac{\lambda}{4\pi d})]
\label{eqn:solution6}
\vspace{-0.05in}
\end{equation}
where $A_{0,k}$ is assumed to be a constant for a specific environment, and the value of $\beta_k = 4$ in case of LOS free space path loss scenario.
%
In reality, $\beta_k$ is dependent upon indoor multipath environment and shadowing effects due to obstructions.

%\vspace{-0.05in}
\subsubsection{Phase}
%\vspace{-0.05in}

For RFID propagation environment involving monostatic readers, the phase information of a received signal, received from $k^{th}$ tag, provided by the reader can be written as $\phi = mod(\phi_p + \phi_o + \phi_{b,k}, 2\pi)$, where $\phi_p = 2kd + \phi_m$ ($k = \frac{2\pi f}{c}$, $f$ = signal frequency and $\phi_m$ phase contribution due to constructive/destructive interference due to multipaths), $\phi_o$ is the phase offset which includes phases of the cables and other reader and antenna components, and $\phi_{b,k}$ is the backscatter phase of the $k^{th}$ tag modulation.

%\vspace{-0.05in}
\subsubsection{Radio Tomographic Imaging (RTI)} \label{rtiintro}
%\vspace{-0.05in}
Our baseline RF imaging approach is similar to the \textit{radio tomographic imaging} (RTI) schemes proposed in \cite{wilson2010radio,wagner2012passive}, which are based on measurement models for RSS attenuation.
%
In these RTI approaches, the area monitored by RF nodes is divided into a grid, where each block of the grid is called a \textit{voxel}.
%
%The basic part of every RTI scheme is to model the changes in attenuation happening inside the area being monitored using the signal strength measurements made at several different nodes of the RTI network. 
%
%Moreover, as motion of an object in an RTI area creates multipaths, the noise in such a dynamic multipath environment also needs to be modeled. In order to achieve this goal, the authors represent the signal strength of a link $i$ as:
%\vspace{-0.05in}
%\begin{equation}
%y_i(t) = P_i - L_i - S_i(t) - F_i(t) - v_i(t)
%\end{equation}
Value of each \textit{voxel} represents the changes in attenuation observed at that voxel. %at any given time.
%
First, RSS values obtained for all possible links are calibrated when there are no obstructions in the monitored area.
%
Afterwards, during the monitoring phase, changes in RSS values of each link are used to determine value of changes in attenuation at each \textit{voxel} to reconstruct image of an obstruction at run-time.
%
\begin{figure*} [htbp]
	\centering
	\captionsetup{justification=centering}
	\subfigure[ \noindent{Image plane intersects first Fresnel zone of a tag-reader pair}]{
		\label{fig:fresnel_zones_1a}
		\includegraphics[width=0.45\textwidth]{figures/Fresnel_Zones_1}%
	}
	\hspace{0.2in}
	\subfigure[ \noindent{Impact of human obstruction on RF propagation paths}]{
		\label{fig:fresnel_zones_1b}
		\includegraphics[width=0.42\textwidth]{figures/Fresnel_Zones_2}%
	}
	\vspace{-0.15in}
	\caption{Intuitions behind using the concept of First Fresnel zones \cite{hristov2000fresnal} for phase based filtering \& our baseline RTI approach} % Tonemaps (Location C and D)}
	\label{fig:fresnel_zones_1}
	\vspace{-0.15in}
\end{figure*}

%
%
%where $P_i$ is transmit power (dB), $S_i$ is shadowing loss due to objects, $F_i(t)$ is loss due to fading, $L_i$ are \textit{static} losses (related to distance, antenna patterns, device inconsistencies, etc.) and $v_i$ is measurement noise. Moreover, shadowing loss $S_i$ for a certain link for a specific time is expressed in terms of attenuation caused in all the voxels as:
%\vspace{-0.05in}
%\begin{equation}
%S_i(t) = \sum_{j=1}^{N} w_{ij}x_j(t)
%\end{equation}
%
%where $x_j(t)$ is attenuation at voxel $j$ at anytime $t$ and $w_{ij}$ is weight-age or contribution of voxel $j$ towards attenuation of link $i$. 
%
%In order to simplify the problem, authors propose to image only the \textit{changing attenuations} between two different times and group the fading and measurement noise into one vector $\mathbf{n}$. 
%
%
This RTI problem can be represented as a linear system of equations, where the changes in RSS of different links $\mathbf{y_{rss}}$ can be written in terms of the changing attenuations $\mathbf{x}$ and an $M \times N$ weight matrix $\mathbf{W}$ (where $M = $ Number of links, $N = $ Number of \textit{voxels} in the grid), specifying the contributions of each link towards the changes observed in attenuation at each different \textit{voxel}, as follows:
\vspace{-0.05in}
\begin{equation}
\mathbf{y_{rss}} = \mathbf{W} \mathbf{x} + \mathbf{n}
\label{eqn:optimzation1}
\vspace{-0.05in}
\end{equation}
where $\mathbf{n}$ corresponds to fading and measurement noise. 
%
To model weight matrix, statistics based measurement models are used to describe linear effect of ``attenuation field'' $\mathbf{x}$ on path loss of different links. 
%
For example, authors in \cite{wilson2010radio,wagner2012passive} use the concept of Fresnel zones \cite{hristov2000fresnal} between two nodes of a RF link, and use imaginary ellipsoids centered at the locations of different RF nodes in the network, to determine weights of different \textit{voxels} in the image plane covering the monitored area.
%
The intuition is, that these ellipsoids determine the LOS path (typically chosen to be the first Fresnel zone) of each respective link, and if a \textit{voxel} is intersected by the LOS path of a link, it will be assigned more weight as compared to the \textit{voxel} which does not fall in LOS.
%
Figure \ref{fig:fresnel_zones_1a} shows an example scenario.
%a) In order to model weight matrix, the authors propose to use a statistical model to describe linear effect of ``attenuation field'' on path loss of different links. In order to determine weights of different voxels in the area, they use an imaginary ellipsoid centered (Fresnel Zone) at the locations of different RF nodes in the network. \textit{The intuition is that ellipsoids will be determining the LOS path of each respective link. If a voxel is within the LOS of a link, it will be assigned more weight as compared to the voxel which does not fall in LOS.} If a voxel is outside the ellipsoid, the assigned weight is 0. However, if the voxel is inside the ellipsoid, the assigned weight is inversely proportional to square root of the distance. \textit{This is because the signals between longer links reflect and diffract around the object being tracked, thus providing less information about the changes in attenuation as compared to a short link.} Let $d$ be distance between two nodes of a certain link $i$, $d_{ij}(1)$ and $d_{ij}(2)$ be distance from center of voxel $j$ to the two nodes of the link $i$ and $\Theta$ be a parameter describing ellipsoid's width. Then the weights can be modeled as:
%\vspace{-0.05in}
%\[
%w_{ij}= 
%\begin{cases}
%\frac{1}{\sqrt{d}},& \text{if } d_{ij}(1) + d_{ij}(2) < d + \Theta\\
%0,              & \text{otherwise}
%\end{cases}
%\]
%
%$\lambda$ is usually chosen so that only the voxels corresponding to line-of-sight (LOS) path are considered. 
%
%b) After modeling of weights for different voxels corresponding to different links, authors propose to model noise as a two-part \textit{log-normal mixture model}. \textit{The reason behind using this model is the similarity of the log-normal distribution with the logarithm of a Rician random variable (often used to model effects of fading in wireless channels)}. 
%
%The authors also derive an error bounds for their proposed models for attenuation weight-age of different voxels corresponding to different links and noise. 
%
To reconstruct image from the RSS difference values obtained for all the links (i.e. $\mathbf{y_{rss}}$), the most straightforward way is to calculate the least-squares solution for the Eq. \ref{eqn:optimzation1} as $\mathbf{x_{LS}} = \mathbf{P}\times\mathbf{y_{rss}}$, where $\mathbf{P} = (\mathbf{W}^T\mathbf{W})^{-1}\mathbf{W}^T$. %(for simplification, we can take $\bigtriangleup x = x$ and $\bigtriangleup y = y$):
%
%\vspace{-0.05in}
%\begin{equation}
%\mathbf{x_{LS}} = (\mathbf{W}^T\mathbf{W})^{-1}\mathbf{W}^T \mathbf{y}
%\label{eqn:solution1}
%\vspace{-0.05in}
%\end{equation}
%
However, the matrix $\mathbf{W}$ is not full rank in case of RTI systems, which makes RTI an \textit{ill-posed inverse problem}. 
%
To handle ill-posedness, different regularization techniques (such as \textit{Tikhonov Regularization} in \cite{wilson2010radio}) are used for minimizing objective function of the original problem (i.e. represented by Eq. \ref{eqn:optimzation1}). 
%
We formulate our RTI problem in a similar manner as mentioned in Eq. \eqref{eqn:optimzation1}.
%
After developing a baseline approach based on a measurement model for RSS attenuation, we propose a deep learning based approach for our monostatic RTI scenario, which allows for automatic and robust estimation of image reconstruction matrix $\mathbf{P}$, when solving for the linear RTI system $\mathbf{x} = \mathbf{P}\times\mathbf{y_{rss}}$.

%\vspace{-0.05in}
%\begin{equation}
%f(\mathbf{x}) = \frac{1}{2}||\mathbf{Wx-y}||^2 + \alpha(||\mathbf{D}_X\mathbf{x}||^2 + ||\mathbf{D}_Y\mathbf{y}||^2)
%\label{eqn:minimization1}
%\end{equation}
%
%where $\mathbf{D}_X$ and $\mathbf{D}_Y$ are different operators in X and Y directions respectively. The solution comes out to be:
%\vspace{-0.05in}
%\begin{equation}
%\mathbf{\hat{x}} = (\mathbf{W}^T\mathbf{W} + \alpha(\mathbf{D}_X^T\mathbf{D}_X + \mathbf{D}_Y^T\mathbf{D}_Y))^{-1}\mathbf{W}^T \mathbf{y}
%\label{eqn:solution2}
%\end{equation}
%
%The total number of multiplications involved in image reconstruction procedure are $\frac{N\times K(K-1)}{2}$, where $N$ = number of voxels and $K$ = number of nodes. The authors have also used the inverse of the covariance matrix $\mathbf{C_x}$ of $\mathbf{\hat{x}}$ as a prior in the technical report of their paper.
%\vspace{-0.05in}
%\begin{equation}
%\mathbf{\hat{x}} = (\mathbf{W}^T\mathbf{W} + \mathbf{C_x}^{-1})^{-1}\mathbf{W}^T \mathbf{y}
%\label{eqn:solution3}
%\end{equation}
%We will discuss later on how we use a combination of these priors to improve our image reconstruction results.

%\begin{figure}[!t]
%	\centering
%	\captionsetup{justification=centering}
%	%	\subfigure[ \noindent{Tonemap N1-N2}]{
%	%		\label{fig:illustration}
%	\includegraphics[width=0.4\textwidth]{figures/rfid_rti.pdf}%}
%	\vspace{-0.1in}
%	\caption{RFID based RTI example \cite{wagner2012passive}} % Tonemaps (Location C and D)
%	\label{fig:rfid_rti}
%	\vspace{-0.15in}
%\end{figure}

==> Kamran/resultsanddiscussion.tex <==
\section{Implementation \& Evaluation}

==> biography.tex <==
\vspace{-0.5in}
\begin{IEEEbiography}
%
[{\includegraphics[width=1in,height=1.10in,clip,keepaspectratio]{figures/kamran}}]{Kamran Ali}
%
is a Ph.D. candidate at Department of Computer Science and Engineering, Michigan State University, USA.
%
He received his B.S. degree in Electrical Engineering and Computer Sciences in 2013, from School of Science and Engineering (SSE) of Lahore University of Management
Sciences (LUMS), Pakistan.
%
He has worked with Hewlett Packard Labs, NEC Laboratories, Nokia Bell Labs and Microsoft's Applied Sciences Group. 
%
His research interests lie in the areas of Sensing Systems, Applied Machine Learning, Wireless Communications, Mobile Computing, Pervasive Computing, Signal Processing, and Internet of Things.
%
\end{IEEEbiography}
%
\vspace{-0.5in}
%
\begin{IEEEbiography}
%
[{\includegraphics[width=1in,height=1.10in,clip,keepaspectratio]{figures/alex}}]{Alex X. Liu}
received his Ph.D. degree in Computer Science from The University of Texas at Austin in 2006, and is a professor at the Department of Computer Science and Engineering, Michigan State University. He received the IEEE \& IFIP William C. Carter Award in 2004, a National Science Foundation CAREER award in 2009, and the Michigan State University Withrow Distinguished Scholar Award in 2011. He has served as an Editor for IEEE/ACM Transactions on Networking, and he is currently an Associate Editor for IEEE Transactions on Dependable and Secure Computing and IEEE Transactions on Mobile Computing, and an Area Editor for Computer Communications. He has served as the TPC Co-Chair for ICNP 2014 and IFIP Networking 2019. He received Best Paper Awards from ICNP-2012, SRDS-2012, and LISA-2010. His research interests focus on networking and security. He is a Fellow of the IEEE.
%
\end{IEEEbiography}
% 
